A Public Image Database for Benchmark of Plant Seedling Classification Algorithms

A database of images of approximately 960 unique plants belonging to 12 species at several growth stages is made publicly available. It comprises annotated RGB images with a physical resolution of roughly 10 pixels per mm. To standardise the evaluation of classification results obtained with the database, a benchmark based on $f_{1}$ scores is proposed. The dataset is available at https://vision.eng.au.dk/plant-seedlings-dataset

==> src/confusionMatrices.tex <==

\begin{figure}[h!]
\subfloat[Nearest Neighbor using full feature set]{
\resizebox{7cm}{!}{ %
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
72 &   0 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Charlock}\\
  3 &  60 &   1 &   3 &   4 &   0 &   0 &   1 & \textbf{b=Cleavers}\\
  1 &   1 &  40 &   8 &   1 &   2 &   0 &   4 & \textbf{c=Shepherd's Purse}\\
  0 &   0 &   3 &  90 &   1 &   3 &   0 &   5 & \textbf{d=Scentless Mayweed}\\
  0 &   9 &   3 &   1 &  45 &   2 &   0 &   2 & \textbf{e=Maize}\\
  0 &   0 &   4 &   8 &   1 &  43 &   0 &   2 & \textbf{f=Sugar beet}\\
  0 &   0 &   0 &   0 &   0 &   0 &  47 &   1 & \textbf{g=Loose Silky-bent}\\
  0 &   0 &   2 &   6 &   0 &   2 &   0 & 113 & \textbf{h=Common Chickweed}\\
\end{tabular}%
}
}
\subfloat[Naive bayes using full feature set]{
\resizebox{7cm}{!}{ %
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
72 &   0 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Charlock}\\
  1 &  61 &   5 &   2 &   1 &   2 &   0 &   0 & \textbf{b=Cleavers}\\
  0 &   2 &  39 &   7 &   3 &   0 &   0 &   6 & \textbf{c=Shepherd's Purse}\\
  0 &   1 &   3 &  85 &   5 &   2 &   0 &   6 & \textbf{d=Scentless Mayweed}\\
  0 &   7 &   4 &   2 &  48 &   0 &   0 &   1 & \textbf{e=Maize}\\
  0 &   0 &   5 &   6 &   1 &  44 &   0 &   2 & \textbf{f=Sugar beet}\\
  0 &   0 &   0 &   0 &   0 &   0 &  48 &   0 & \textbf{g=Loose Silky-bent}\\
  0 &   0 &   6 &   2 &   3 &   3 &   0 & 109 & \textbf{h=Common Chickweed}\\
\end{tabular} %
}
}

\subfloat[Random Forest using full feature set]{
\resizebox{7cm}{!}{ %
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
71 &   1 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Charlock}\\
  1 &  62 &   3 &   2 &   2 &   2 &   0 &   0 & \textbf{b=Cleavers}\\
  0 &   1 &  43 &   6 &   2 &   1 &   0 &   4 & \textbf{c=Shepherd's Purse}\\
  0 &   0 &   1 &  95 &   3 &   0 &   0 &   3 & \textbf{d=Scentless Mayweed}\\
  1 &   6 &   1 &   3 &  49 &   0 &   0 &   2 & \textbf{e=Maize}\\
  0 &   0 &   3 &   8 &   2 &  43 &   0 &   2 & \textbf{f=Sugar beet}\\
  0 &   0 &   0 &   0 &   0 &   0 &  48 &   0 & \textbf{g=Loose Silky-bent}\\
  0 &   0 &   2 &   4 &   0 &   2 &   0 & 115 & \textbf{h=Common Chickweed}\\
\end{tabular}%
}
}
\subfloat[Nearest Neighbor using reduced feature set]{
\resizebox{7cm}{!}{ %
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 72 &   0 &   0 &   0 &   0 &   1 &   0 &   0 & \textbf{a=Charlock}\\
  1 &  61 &   2 &   3 &   4 &   1 &   0 &   0 & \textbf{b=Cleavers}\\
  0 &   1 &  45 &   8 &   1 &   1 &   0 &   1 & \textbf{c=Shepherd's Purse}\\
  0 &   0 &   1 &  94 &   3 &   2 &   0 &   2 & \textbf{d=Scentless Mayweed}\\
  0 &   5 &   0 &   4 &  45 &   4 &   0 &   4 & \textbf{e=Maize}\\
  1 &   0 &   3 &   6 &   2 &  44 &   0 &   2 & \textbf{f=Sugar beet}\\
  0 &   0 &   0 &   0 &   0 &   0 &  47 &   1 & \textbf{g=Loose Silky-bent}\\
  0 &   0 &   3 &   3 &   0 &   0 &   0 & 117 & \textbf{h=Common Chickweed}\\
\end{tabular} %
}
}

\subfloat[Naive bayes using reduced feature set]{
\resizebox{7cm}{!}{ %
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 71 &   1 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Charlock}\\
  0 &  61 &   4 &   1 &   3 &   2 &   0 &   1 & \textbf{b=Cleavers}\\
  0 &   1 &  31 &  10 &   2 &   5 &   0 &   8 & \textbf{c=Shepherd's Purse}\\
  0 &   1 &   3 &  81 &   7 &   4 &   0 &   6 & \textbf{d=Scentless Mayweed}\\
  0 &   6 &   6 &   6 &  41 &   1 &   1 &   1 & \textbf{e=Maize}\\
  0 &   0 &   6 &   8 &   1 &  42 &   0 &   1 & \textbf{f=Sugar beet}\\
  0 &   0 &   0 &   0 &   0 &   0 &  48 &   0 & \textbf{g=Loose Silky-bent}\\
  0 &   0 &   3 &   1 &   7 &   5 &   0 & 107 & \textbf{h=Common Chickweed}\\
\end{tabular}%
}
}
\subfloat[Random Forest using full feature set]{
\label{tab:RandForestReduces}
\resizebox{7cm}{!}{ %
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 71 &   1 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Charlock}\\
  0 &  65 &   2 &   2 &   1 &   2 &   0 &   0 & \textbf{b=Cleavers}\\
  0 &   0 &  41 &   8 &   1 &   1 &   0 &   6 & \textbf{c=Shepherd's Purse}\\
  0 &   0 &   0 &  95 &   4 &   0 &   0 &   3 & \textbf{d=Scentless Mayweed}\\
  0 &   5 &   2 &   4 &  48 &   1 &   0 &   2 & \textbf{e=Maize}\\
  0 &   0 &   3 &   8 &   1 &  42 &   0 &   4 & \textbf{f=Sugar beet}\\
  0 &   0 &   0 &   0 &   0 &   0 &  47 &   1 & \textbf{g=Loose Silky-bent}\\
  0 &   0 &   3 &   2 &   0 &   1 &   0 & 117 & \textbf{h=Common Chickweed}\\
\end{tabular} %
}
}
\end{figure}



==> src/confusionMatricesTables.tex <==

\begin{table}[h!]
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 72 &   0 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Agersennep}\\
  1 &  61 &   5 &   2 &   1 &   2 &   0 &   0 & \textbf{b=Burresnerre}\\
  0 &   2 &  38 &   7 &   3 &   0 &   0 &   7 & \textbf{c=Hyrdetaske}\\
  0 &   1 &   2 &  87 &   4 &   3 &   0 &   5 & \textbf{d=Lughløs}\\
  0 &   7 &   3 &   2 &  49 &   0 &   0 &   1 & \textbf{e=Majs}\\
  0 &   0 &   5 &   6 &   1 &  44 &   0 &   2 & \textbf{f=Sukkerroe}\\
  0 &   0 &   0 &   0 &   0 &   0 &  48 &   0 & \textbf{g=Vinaks}\\
  0 &   0 &   4 &   1 &   4 &   3 &   0 & 111 & \textbf{h=kamille Fuglegræs}\\
\end{tabular}
\end{table}



\begin{table}[h!]
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 72 &   0 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Agersennep}\\
  3 &  60 &   1 &   3 &   4 &   0 &   0 &   1 & \textbf{b=Burresnerre}\\
  1 &   1 &  40 &   8 &   1 &   2 &   0 &   4 & \textbf{c=Hyrdetaske}\\
  0 &   0 &   3 &  90 &   1 &   3 &   0 &   5 & \textbf{d=Lughløs}\\
  0 &   9 &   3 &   1 &  45 &   2 &   0 &   2 & \textbf{e=Majs}\\
  0 &   0 &   4 &   8 &   1 &  43 &   0 &   2 & \textbf{f=Sukkerroe}\\
  0 &   0 &   0 &   0 &   0 &   0 &  47 &   1 & \textbf{g=Vinaks}\\
  0 &   0 &   2 &   6 &   0 &   2 &   0 & 113 & \textbf{h=kamille Fuglegræs}\\
\end{tabular}
\caption{Nearest Neighbor: mean f-measure of 0.8476 with a 95\% confidence interval of [0.8252:0.8713]}
\end{table}


\begin{table}[h!]
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 72 &   0 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Agersennep}\\
  1 &  61 &   5 &   2 &   1 &   2 &   0 &   0 & \textbf{b=Burresnerre}\\
  0 &   2 &  39 &   7 &   3 &   0 &   0 &   6 & \textbf{c=Hyrdetaske}\\
  0 &   1 &   3 &  85 &   5 &   2 &   0 &   6 & \textbf{d=Lughløs}\\
  0 &   7 &   4 &   2 &  48 &   0 &   0 &   1 & \textbf{e=Majs}\\
  0 &   0 &   5 &   6 &   1 &  44 &   0 &   2 & \textbf{f=Sukkerroe}\\
  0 &   0 &   0 &   0 &   0 &   0 &  48 &   0 & \textbf{g=Vinaks}\\
  0 &   0 &   6 &   2 &   3 &   3 &   0 & 109 & \textbf{h=kamille Fuglegræs}\\
\end{tabular}
\caption{Naive bayes : mean f-measure of 0.8509 with a 95\% confidence interval of [0.8200:0.8787]}
\end{table}


\begin{table}[h!]
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 71 &   1 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Agersennep}\\
  1 &  62 &   3 &   2 &   2 &   2 &   0 &   0 & \textbf{b=Burresnerre}\\
  0 &   1 &  43 &   6 &   2 &   1 &   0 &   4 & \textbf{c=Hyrdetaske}\\
  0 &   0 &   1 &  95 &   3 &   0 &   0 &   3 & \textbf{d=Lughløs}\\
  1 &   6 &   1 &   3 &  49 &   0 &   0 &   2 & \textbf{e=Majs}\\
  0 &   0 &   3 &   8 &   2 &  43 &   0 &   2 & \textbf{f=Sukkerroe}\\
  0 &   0 &   0 &   0 &   0 &   0 &  48 &   0 & \textbf{g=Vinaks}\\
  0 &   0 &   2 &   4 &   0 &   2 &   0 & 115 & \textbf{h=kamille Fuglegræs}\\
\end{tabular}
\caption{Random Forest: mean f-measure of 0.8825 with a 95\% confidence interval of [0.8628:0.9116]}
\end{table}

\begin{table}[h!]
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 72 &   0 &   0 &   0 &   0 &   1 &   0 &   0 & \textbf{a=Agersennep}\\
  1 &  61 &   2 &   3 &   4 &   1 &   0 &   0 & \textbf{b=Burresnerre}\\
  0 &   1 &  45 &   8 &   1 &   1 &   0 &   1 & \textbf{c=Hyrdetaske}\\
  0 &   0 &   1 &  94 &   3 &   2 &   0 &   2 & \textbf{d=Lughløs}\\
  0 &   5 &   0 &   4 &  45 &   4 &   0 &   4 & \textbf{e=Majs}\\
  1 &   0 &   3 &   6 &   2 &  44 &   0 &   2 & \textbf{f=Sukkerroe}\\
  0 &   0 &   0 &   0 &   0 &   0 &  47 &   1 & \textbf{g=Vinaks}\\
  0 &   0 &   3 &   3 &   0 &   0 &   0 & 117 & \textbf{h=kamille Fuglegræs}\\
\end{tabular}
\caption{Nearest Neighbor: mean f-measure of 0.8828 with a 95\% confidence interval of [0.8568:0.9093] using reduced feature set}
\end{table}


\begin{table}[h!]
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 71 &   1 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Agersennep}\\
  0 &  61 &   4 &   1 &   3 &   2 &   0 &   1 & \textbf{b=Burresnerre}\\
  0 &   1 &  31 &  10 &   2 &   5 &   0 &   8 & \textbf{c=Hyrdetaske}\\
  0 &   1 &   3 &  81 &   7 &   4 &   0 &   6 & \textbf{d=Lughløs}\\
  0 &   6 &   6 &   6 &  41 &   1 &   1 &   1 & \textbf{e=Majs}\\
  0 &   0 &   6 &   8 &   1 &  42 &   0 &   1 & \textbf{f=Sukkerroe}\\
  0 &   0 &   0 &   0 &   0 &   0 &  48 &   0 & \textbf{g=Vinaks}\\
  0 &   0 &   3 &   1 &   7 &   5 &   0 & 107 & \textbf{h=kamille Fuglegræs}\\
\end{tabular}
\caption{Naive bayes : mean f-measure of 0.8062 with a 95\% confidence interval of [0.7763:0.8444] using reduced feature set}
\end{table}



\begin{table}[h!]
\small
\begin{tabular}{c c c c c c c c r}
\textbf{  a} & \textbf{  b} & \textbf{  c} & \textbf{  d} & \textbf{  e} & \textbf{  f} & \textbf{  g} & \textbf{  h} & \slashbox{\textbf{Predicted class}}{\textbf{True class}}\\
 71 &   1 &   1 &   0 &   0 &   0 &   0 &   0 & \textbf{a=Agersennep}\\
  0 &  65 &   2 &   2 &   1 &   2 &   0 &   0 & \textbf{b=Burresnerre}\\
  0 &   0 &  41 &   8 &   1 &   1 &   0 &   6 & \textbf{c=Hyrdetaske}\\
  0 &   0 &   0 &  95 &   4 &   0 &   0 &   3 & \textbf{d=Lughløs}\\
  0 &   5 &   2 &   4 &  48 &   1 &   0 &   2 & \textbf{e=Majs}\\
  0 &   0 &   3 &   8 &   1 &  42 &   0 &   4 & \textbf{f=Sukkerroe}\\
  0 &   0 &   0 &   0 &   0 &   0 &  47 &   1 & \textbf{g=Vinaks}\\
  0 &   0 &   3 &   2 &   0 &   1 &   0 & 117 & \textbf{h=kamille Fuglegræs}\\
\end{tabular}
\caption{Random Forest: mean f-measure of 0.8796 with a 95\% confidence interval of [0.8518:0.9037] using reduced feature set}
\end{table}

